DPA-Net: Structured 3D Abstraction from Sparse Views via Differentiable Primitive Assembly

We present a differentiable rendering framework to learn structured 3D abstractions in the form of primitive assemblies from sparse RGB images capturing a 3D object. By leveraging differentiable volume rendering, our method does not require 3D supervision. Architecturally, our network follows the general pipeline of an image-conditioned neural radiance field (NeRF) exemplified by pixelNeRF for color prediction. As our core contribution, we introduce differential primitive assembly (DPA) into NeRF to output a 3D occupancy field in place of density prediction, where the predicted occupancies serve as opacity values for volume rendering. Our network, coined DPA-Net, produces a union of convexes, each as an intersection of convex quadric primitives, to approximate the target 3D object, subject to an abstraction loss and a masking loss, both defined in the image space upon volume rendering. With test-time adaptation and additional sampling and loss designs aimed at improving the accuracy and compactness of the obtained assemblies, our method demonstrates superior performance over state-of-the-art alternatives for 3D primitive abstraction from sparse views.

==> tables/color.tex <==
\begin{table}[htbp]
\centering
%\small
\caption{Quantitative comparisons for rendered images on the ShapeNet chair benchmark for 3 input views. }
\begin{tabular}{l|c|c|} \hline
Method & PSNR $\!\uparrow$ & SSIM $\!\uparrow$ \\  \hline \hline
pixelNeRF & 27.85 & 0.963 \\ \hline 
Ours & 27.30 & 0.960 \\ \hline 
\end{tabular}
\label{tab:color_chair}
\end{table}
\vspace{-5pt}

==> tables/ins_seg.tex <==
\begin{table}\centering
\caption{Instance segmentation comparison on the SRN chair category.}
%\begin{tabular}{@{}cccc@{}}

 \begin{tabular}{|l| c| c| c| c|}
    % \toprule
     \hline
 Methods & mIoU $\uparrow$ & MV & 3D & PT\\
    % \midrule
    %     \addlinespace[5pt]
    \hline \hline
  EMS & 0.314   & -  & \checkmark & -\\
  DBW & 0.450   & \checkmark  & - & -\\
  Ours & \textbf{0.728}  & \checkmark  & - & \checkmark\\
  \hline
  
\end{tabular}
\label{tab:ins_seg}
\end{table}
